Marine Autonomous Vehicle Fleet Scheduling to Maximise Scientific Impact

The marine science community increasingly relies on Marine Autonomous Vehicles (MAVs) to collect the critical environmental data required to understand global ocean systems. However, as these operations scale, manually routing and planning large autonomous fleets becomes exponentially complex and time-consuming. To address this, we propose a mixed-integer linear programming (MILP) model designed to automate and optimise MAV deployment schedules. The model accounts for strict operational constraints, including battery capacities and time windows for data collection, while aiming to maximise total data collection and minimise both the number of deployed vehicles and their energy consumption. A key novelty of this framework is integrating conventional ship itineraries, allowing MAVs to support vessels with mid-mission battery swapping or accelerated transit between waypoints. Computational experiments demonstrate that the model is highly scalable, solving routing problems for fleets of dozens of MAVs in seconds, and scaling to hundreds of vehicles in only a few minutes. Beyond operational scheduling, the framework serves as a robust simulation tool for evaluating 'what-if' scenarios and analysing the impact of varying parameters on deployment strategies. Finally, the solution generates a suite of visualisations designed to enhance explainability and support strategic decision-making for stakeholders.

==> section_case_studies/results.tex <==
\subsection{Results}


\subsubsection{Deployment around Rothera, Antarctica} 
\label{sssec:rothera_results}
All the task requirements were covered in this case study. Moreover, the model succeeded in sparing one MAV of type "\textit{Slocum - CTD+optode+PAR+Ecopuck}".
In addition to the activities on the timeline in Figure \ref{fig:timeline_case_study1}, we can also see in almost every MAV some idle times. This is explained by differences in time windows and the short distances between locations.
These idle times can be exploited to conduct opportunistic science and maximise the scientific gain from the same deployment. 
The histogram in Figure \ref{fig:histogram_case_study1}, via its non-uniform distribution, indicates that the deployed MAVs could be better utilised during their idle periods.

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{timeline_case_study1.png}
    \caption{Timeline of MAV activities for the deployment around Rothera}
    \label{fig:timeline_case_study1}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{histogram_case_study1.png}
    \caption{Amount of science data collected during the deployment around Rothera for each sensor}
    \label{fig:histogram_case_study1}
\end{figure}

\subsubsection{Southern Atlantic/Antarctica}
The RRS SDA itinerary considered in this use case is added to the timeline alongside the deployed MAVs. Only the ship tasks are added to indicate the time windows during which the MAVs are assigned for charging or transit.

From the timeline in Figure \ref{fig:timeline_case_study2}, we can notice that many MAVs are assigned to the SDA.
Knowing that the minimum duration of stay at the ship is one day (set in the input parameters), the MAV assignment to the ship is for battery swapping/charging when the MAV comes to the ship and leaves in the same time window, while it is for transiting when it leaves in a different time window.

The heatmap in Figure \ref{fig:heatmap_case_study2} shows that the task scheduled in the research station S1 for the MAV type "\textit{Slocum - CTD+microstructure+ADCP}" is missing half of the required MAVs. Since the model returns the optimal solution, this case study cannot have all the reviews completed at 100\%. Instead, a different assignment of MAVs might be generated by, for example, assigning a higher task weight to some tasks.

To assess the usefulness of a research ship in similar use cases, we ran the same example, excluding the ship from the model. Moreover, while the initial case study is given with a diverse battery level for the MAVs, we set all batteries to 100\% in this variation to reduce ship dependency. Figure \ref{fig:heatmap_case_study2_noship_100} shows that even with full batteries at the beginning of the deployment, the science coverage is still lower than in the original case study.

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{timeline_case_study2.png}
    \caption{Timeline of MAV activities for the deployment in the Southern Atlantic}
    \label{fig:timeline_case_study2}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{heatmap_case_study2.png}
    \caption{Heatmap of completion rates of task requirements for the deployment in the Southern Atlantic}
    \label{fig:heatmap_case_study2}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{heatmap_case_study2_noship_100.png}
    \caption{Heatmap of completion rates of task requirements for the deployment in the Southern Atlantic, without soliciting a research ship and deploying all the MAVs at 100\% of battery}
    \label{fig:heatmap_case_study2_noship_100}
\end{figure}

\subsubsection{United Kingdom Large Scale Deployment}
To illustrate the complex coordination of assets, we create a series of snapshots throughout the plan returned by the solver, as shown in Figure \ref{fig:timelocations_case_study3}. For each panel, the locations of the assets on that date are shown by coloured circles, where the colour represents the asset type, and lines represent the path the asset has taken over the last 30 days. We can observe in the first couple of panels that MAVs are predominantly operating in the North Sea (Panels a and b). However, as the ship's itinerary progresses, the autonomous vehicles transit into the Atlantic Ocean to complete science surveys, with some assets rendezvousing with the ship, being collected and dropped off closer to Scotland when the ship transits back to Harwich (Panels c and d). The remaining assets in the Atlantic Ocean transit back to Scotland for collection (Panel c–e). 

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{timelocations_case_study3.png}
    \caption{Time evolution of assets in plan. Panels (a) – (e). Each circle represents the asset location on the panel date, with the tails representing its path over the last 30 days, and colours indicating the asset type. The blue boxes represent the science locations and the red boxes the ship waypoint locations.}
    \label{fig:timelocations_case_study3}
\end{figure}
